Possible Relations between Brightest Central Galaxies and Their Host Galaxies Clusters and Groups

The r-band of the Sloan Digital Sky Survey (SDSS) for 17,924 brightest cluster galaxies (BCGs) in clusters and groups within 0.02 z 0.20 are used to study possible environmental relations affecting the nature of these galaxies. We find a correlation between BCGs physical properties (the effective radius (Re ), absolute magnitude and central velocity dispersion ({\sigma}0 )) and their host groups and clusters velocity dispersion ({\sigma}cl ). This type of relations suggests that the most massive groups or clusters host larger central galaxies. On the other hand, the {\sigma}0 /{\sigma}cl ratio as a function of {\sigma}cl is consistent with [10].

==> lost-paragraphs.tex <==

From table named \textit{Galaxy} we extracted the following parameters: de Vaucouleurs angular radius ($r_{dev}$) in arcsec, which is defined to be the same as the effective radius, de Vaucouleurs axis ratio (b/a), extinction (A), and composite Model (cModel) magnitude, that is a linear combination of de Vaucouleurs and model magnitudes. From table \textit{Photoz}, we extracted the k-correction at $z = 0$ and the luminosity distance (\textit{D$_L$}). We extracted velocity dispersion ($\sigma$) in km s$^{-1}$ and spectroscopic redshift ($z$) from table named \textit{SpecObj}. 

In our study, the surface brightness profile of central galaxies is fitted by the de Vaucouleurs' model, that seems to be a good fit to the surface brightness profiles of elliptical galaxies in the SDSS sample. Also, the de Vaucouleurs’ model is widely used in literature for studying elliptical galaxies \citep{Bernardi03b, Hou15}. On the other side, the S\'{e}rsic model is used extensively in galaxy studies. Pure S\'{e}rsic model fits might be more suitable for studying galaxy colors such that a bulge+disk model fits are favored for studies of bulge/disk colors \citep{Simard2011}. Also \cite{Meert2015} preferred the S\'{e}rsic+Exponential model for both studying the structure of the galaxies (i.e. one versus two components) and for determining the total size and magnitude of galaxies.

The morphological classification of our galaxies is obtained from the  \textit{zooSpec} table, which is concerned with morphological classifications of spectroscopic galaxies from Galaxy Zoo project in SDSS-DR16. The Galaxy Zoo 
project provides visual morphological classifications for about one million galaxies, contributed by hundreds of thousands of volunteers. The Galaxy Zoo classifies objects into elliptical, spiral and uncertain. The project is described in \citet{Lintott08} and the data release is described in \citet{Lintott2011}. 

We cross-matched our sample of 55,968 brightest central galaxies with \textit{zooSpec} table and  
obtained

 We extracted cModel magnitude and extinction from \textit{Galaxy} table, while k-correction values and \textit{D$_L$} are extracted from \textit{Photoz} table. 
 
 

